Boosting Discriminative Visual Representation Learning with Scenario-Agnostic Mixup

Mixup is a well-known data-dependent augmentation technique for DNNs, consisting of two sub-tasks: mixup generation and classification. However, the recent dominant online training method confines mixup to supervised learning (SL), and the objective of the generation sub-task is limited to selected sample pairs instead of the whole data manifold, which might cause trivial solutions. To overcome such limitations, we comprehensively study the objective of mixup generation and propose \textbf{S}cenario-\textbf{A}gnostic \textbf{Mix}up (SAMix) for both SL and Self-supervised Learning (SSL) scenarios. Specifically, we hypothesize and verify the objective function of mixup generation as optimizing local smoothness between two mixed classes subject to global discrimination from other classes. Accordingly, we propose $\eta$-balanced mixup loss for complementary learning of the two sub-objectives. Meanwhile, a label-free generation sub-network is designed, which effectively provides non-trivial mixup samples and improves transferable abilities. Moreover, to reduce the computational cost of online training, we further introduce a pre-trained version, SAMix$^\mathcal{P}$, achieving more favorable efficiency and generalizability. Extensive experiments on nine SL and SSL benchmarks demonstrate the consistent superiority and versatility of SAMix compared with existing methods.

==> Tabs/analysis_loss.tex <==

\begin{table}[H]
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|cc|cc}
    \toprule
                   & \multicolumn{2}{c|}{STL-10\wbfup{+0.0}}               & \multicolumn{2}{c}{Tiny ImageNet} \\
    Loss function  & SL\wbfup{+0.00}           & CL\wbfup{+0.00}           & SL\wbfup{+0.00}           & CL\wbfup{+0.00}  \\ \hline
    \gray{Mixup}   & \gray{78.94}\wbfup{+0.00} & \gray{84.51}\wbfup{+0.00} & \gray{63.39}\wbfup{+0.00} & \gray{41.24}\wbfup{+0.00} \\
    CE (L)         & \bf{82.14}\grybfup{+0.00} & \bf{85.95}\grybfup{+0.00} & \bf{68.56}\grybfup{+0.00} & \bf{43.11}\grybfup{+0.00} \\
    CE (PL), K=100 & 81.47\rbfup{-0.67}        & 85.56\rbfup{-0.39}        & 67.12\rbfup{-1.44}        & 41.97\rbfup{-1.14}  \\
    CE (PL), K=200 & 81.65\rbfup{-0.49}        & 85.64\rbfup{-0.31}        & 67.39\rbfup{-1.17}        & 42.36\rbfup{-0.75}  \\
    pBCE (L)       & 81.96\rbfup{-0.18}        & 85.78\rbfup{-0.17}        & 67.84\rbfup{-0.72}        & 42.70\rbfup{-0.41}  \\ \hline
    BCE            & 80.50\grybfup{+0.00}      & 85.25\grybfup{+0.00}      & 66.02\grybfup{+0.00}      & 41.28\grybfup{+0.00}  \\
    infoNCE        & 80.67\dgbfup{+0.17}       & 85.37\dgbfup{+0.12}       & 66.36\dgbfup{+0.34}       & 41.93\dgbfup{+0.65}  \\
    infoNCE (PL)   & 81.04\dgbfup{+0.54}       & 85.53\dgbfup{+0.28}       & 66.79\dgbfup{+0.77}       & 42.10\dgbfup{+0.82}  \\
    infoNCE (L)    & \bf{81.28}\dgbfup{+0.78}  & \bf{85.64}\dgbfup{+0.39}  & \bf{67.07}\dgbfup{+1.05}  & \bf{42.31}\dgbfup{+1.03}  \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-6pt}
    \caption{Analysis of the loss functions for training MixBlock. L and PL denote ground-truth labels and pseudo labels respectively. K is the number cluster assigned to the clustering algorithm (ODC). The upper part of the table demonstrates the analysis for parametric losses, while the lower part is for non-parametric losses.}
    \label{tab:analysis_loss}
\end{table}


==> Tabs/analysis_mixup.tex <==

\begin{table}[h]
\vspace{-4pt}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|c|c}
    \toprule
    Property & Instance-level mixup                                      & Class-level mixup                                       \\ \hline
    Local    & $(1-\lambda) I(x_{m}^*, x_i) = \lambda I(x_{m}^*, x_j)$   & $(1-\lambda) I(x_{m}^*, y_i) = \lambda I(x_{m}^*, y_j)$ \\
    Global   & $I(x_{m}^*, x_{k}) = 0, \forall k, k\neq i, k\neq j.$     & $I(x_{m}^*, y_{c}) = 0, \forall c, y_c\neq y_i, y_c\neq y_j.$    \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-8pt}
    \caption{Properties of learning objectives of mixup generation.}
    \label{tab:analysis_mixup}
\end{table}


==> Tabs/app_sl_cifar.tex <==
\begin{table}[H]
\resizebox{0.80\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc}
    \toprule
                     & \multicolumn{3}{c|}{R-18}                   & \multicolumn{3}{c}{RX-50} \\ 
    Method           & 400ep        & 800ep        & 1200ep        & 400ep        & 800ep        & 1200ep  \\ \hline
    Vanilla          & 77.73        & 78.04        & 78.55         & 80.24        & 81.09        & 81.32  \\
    MixUp            & 79.34        & 79.12        & 79.24         & 82.54        & 82.10        & 81.77  \\
    CutMix           & 79.58        & 78.17        & 78.29         & 82.34        & 81.67        & 81.27  \\
    ManifoldMix      & 80.18        & 80.35        & 80.21         & 82.56        & 82.88        & 83.28  \\
    SaliencyMix      & 79.64        & 79.12        & 77.66         & 79.28        & 81.53        & 81.31  \\
    FMix$^*$         & 79.91        & 79.69        & 79.50         & 79.79        & 81.90        & 81.22  \\
    PuzzleMix$^\dag$ & 80.22        & 80.43        & 80.64         & 82.84        & 82.57        & 82.85  \\
    ResizeMix$^*$    & 79.19        & 80.01        & 79.23         & 80.96        & 81.82        & 81.85  \\
    AutoMix$^*$      & \blue{81.78} & \blue{82.04} & \blue{81.95}  & \blue{83.32} & \blue{83.64} & \blue{83.80}  \\
    \bf{SAMix}       & \bf{81.97}   & \bf{82.30}   & \bf{82.41}    & \bf{84.27}   & \bf{84.42}   & \bf{84.31}  \\ \hline
    Gain             & \gfn{+0.19}  & \gfn{+0.26}  & \gfn{+0.46}   & \gfn{+0.95}  & \gfn{+0.78}  & \gfn{+0.51}  \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-4pt}
    \caption{Top-1 accuracy (\%) of image classification on CIFAR-100.}
    % \vspace{-10pt}
    \label{tab:app_sl_cifar}
\end{table}


==> Tabs/app_sl_imagenet.tex <==

\begin{table}[h]
\centering
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
    Method           & R-18         & R-34         & R-50         & R-101        & RX-101 \\ \hline
    Vanilla          & 70.04        & 73.85        & 76.93        & 78.18        & 78.71  \\
    MixUp            & 69.98        & 73.97        & 77.12        & 78.97        & 79.98  \\
    CutMix           & 68.95        & 73.14        & 77.07        & 78.96        & 80.42  \\
    ManifoldMix      & 69.98        & 73.98        & 76.91        & 79.02        & 79.93  \\
    SaliencyMix      & 69.12        & 73.24        & 77.15        & 79.01        & 80.27  \\
    FMix$^*$         & 68.37        & 73.04        & 77.20        & 79.09        & 80.06  \\
    AugMix$^\dag$    & -            & -            & 77.23        & -            & -  \\
    PuzzleMix$^\dag$ & 70.12        & 74.26        & 77.54        & 79.43        & 80.63  \\
    Co-Mixup$^\dag$  & -            & -            & 77.60        & -            & -  \\
    SuperMix$^\dag$  & -            & -            & 77.61        & -            & -  \\
    ResizeMix$^*$    & 69.50        & 73.88        & 77.57        & 79.27        & 80.55  \\
    AutoMix$^*$      & \blue{70.47} & \blue{74.52} & \blue{77.91} & \blue{79.84} & \blue{80.87}  \\
    \bf{SAMix}       & \bf{70.85}   & \bf{74.96}   & \bf{78.11}   & \bf{80.03}   & \bf{81.02}  \\ \hline
    Gain             & \gfn{+0.38}  & \gfn{+0.34}  & \gfn{+0.20}  & \gfn{+0.19}  & \gfn{+0.15}  \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-4pt}
    \caption{Top-1 accuracy (\%) on ImageNet-1k training 100-epoch based on various network architectures.}
    % \vspace{-10pt}
    \label{tab:app_sl_imagenet}
\end{table}


==> Tabs/sl_cifar_tiny.tex <==
%%% update 12.23 %%%
\begin{table}[b]
\vspace{-8pt}
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cc|ccc|cc}
    \toprule
                   & \multicolumn{2}{c|}{CIFAR-10} & \multicolumn{3}{c|}{CIFAR-100}             & \multicolumn{2}{c}{Tiny}     \\
    Method         & R-18         & RX-50          & R-18         & RX-50        & WRN-28-8     & R-18         & RX-50         \\ \hline
    Vanilla        & 95.50        & 96.23          & 78.04        & 81.09        & 81.63        & 61.68        & 65.04         \\
    Mixup          & 96.62        & 97.30          & 79.12        & 82.10        & 82.82        & 63.86        & 66.36         \\
    CutMix         & 96.68        & 97.01          & 78.17        & 81.67        & 84.45        & 65.53        & 66.47         \\
    ManifoldMix    & 96.71        & 97.33          & 80.35        & 82.88        & 83.24        & 64.15        & 67.30         \\
    SaliencyMix    & 96.53        & 97.18          & 79.12        & 81.53        & 84.35        & 64.60        & 66.55         \\
    FMix$^*$       & 96.58        & 96.76          & 79.69        & 81.90        & 84.21        & 63.47        & 65.08         \\
    PuzzleMix      & 97.10        & 97.27          & 80.43        & 82.57        & 85.02        & 65.81        & 66.92         \\
    ResizeMix$^*$  & 96.76        & 97.21          & 80.01        & 81.82        & 84.87        & 63.74        & 65.87         \\
    AutoMix$^*$    & \blue{97.34} & \blue{97.65}   & \blue{82.04} & \blue{83.64} & \blue{85.18} & \blue{67.33} & \blue{70.72}  \\
    \bf{SAMix}     & \bf{97.50}   & \bf{97.93}     & \bf{82.30}   & \bf{84.42}   & \bf{85.50}   & \bf{68.89}   & \bf{72.18}    \\ \hline
    Gain           & \gfn{+0.16}  & \gfn{+0.28}    & \gfn{+1.24}  & \gfn{+0.27}  & \gfn{+0.32}  & \gfn{+1.56}  & \gfn{+1.46}   \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-8pt}
    \caption{Top-1 Acc (\%) of supervised image classification on CIFAR-10/100 and Tiny.}
    \label{tab:sl_cifar_tiny}
\end{table}


==> Tabs/ssl_detection.tex <==
\begin{table}[H]
\resizebox{\linewidth}{!}{
    \begin{tabular}{ll|ccc}
    \toprule
    CL Method          & mixup method       & AP          & AP$_{50}$   & AP$_{75}$  \\ \hline
    MoCo.V2            & -                  & 56.9        & 82.2        & 63.4  \\
    MoCo.V2            & Mixup              & 57.4        & 82.5        & 64.0  \\
    MoCo.V2            & CutMix             & 57.3        & 82.7        & 64.1  \\
    MoCHi$^{\dag}$     & $input$+$latent$   & 57.1        & 82.7        & 64.1  \\
    i-Mix$^{\dag}$     & $input$+$latent$   & 57.5        & 82.7        & \blue{64.2}  \\
    UnMix$^{\ddagger}$ & $input$+$latent$   & \blue{57.7} & \blue{83.0} & \bf{64.3}    \\
    WBSIM$^{\ddagger}$ & $input$            & 57.4        & 82.8        & \blue{64.2}  \\
    MoCo.V2            & \bf{SAMix-I}       & \bf{57.8}   & \bf{83.1}   & \bf{64.3}    \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-6pt}
    \caption{Transferring to detection with Faster R-CNN on VOC07+12.}
    \label{tab:detection}
\end{table}

